HRTF Individualization: A Survey

The individuality of head-related transfer functions (HRTFs) is a key issue for binaural synthesis. While, over the years, a lot of work has been accomplished to propose end-user-friendly solutions to HRTF personalization, it remains a challenge. In this article we establish a state-of-the-art of that work. We classify the various proposed methods, review their respective advantages and disadvantages, and, above all, methodically check if and how the perceptual validity of the resulting HRTFs was assessed.

==> tabMethodsOverview.tex <==
% Definitions
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newlength{\localcolwidth} \setlength{\localcolwidth}{.22\textwidth}

% Table
\begin{table*}
\centering

\begin{tabular}{L{\localcolwidth}
                L{\localcolwidth}
                L{\localcolwidth}
                L{\localcolwidth}}
\toprule
	& Necessary equipment
	& Measurement time (order of magnitude)
	& Processing time (order of magnitude) \\ \midrule
Acoustic Measurement
	& Anechoic room, loudspeakers, motorized structure, etc.
	& $20 \textnormal{mn} - 2 \textnormal{h} 30$  
	& $\sim 1 \textnormal{mn}$ \\ \midrule
Numerical Simulation
	& 3D scanner
	& $\sim 10 \textnormal{mn}$ 
	& $\sim 1 \textnormal{h} - 10 \textnormal{h}$ \\ \midrule
Indirect Individualization from Morphology
	& Camera
	& $\sim 10 \textnormal{s}$ 
	& $\sim 10 \textnormal{s}$ \\ \midrule
Indirect Individualization from Perceptual Feedback 
	& Smartphone, tablet or computer
	& $0$
	& $\sim 10 \textnormal{mn} - 1 \textnormal{h}$  % $\sim$ 10mn - $\infty$  %(selection) %(adaptation direction by direction) 
	\\ \bottomrule
	
\end{tabular}

\caption{Overview of the constraints for the major HRTF individualization approaches}
\label{tabMethodsOverview}	
	
\end{table*}
